HelixTrack: Event-Based Tracking and RPM Estimation of Propeller-like Objects

Safety-critical perception for unmanned aerial vehicles and rotating machinery requires microsecond-latency tracking of fast, periodic motion under egomotion and strong distractors. Frame-based and event-based trackers drift or break on propellers because periodic signatures violate their smooth-motion assumptions. We tackle this gap with HelixTrack, a fully event-driven method that jointly tracks propeller-like objects and estimates their rotations per minute (RPM). Incoming events are back-warped from the image plane into the rotor plane via a homography estimated on the fly. A Kalman Filter maintains instantaneous estimates of phase. Batched iterative updates refine the object pose by coupling phase residuals to geometry. To our knowledge, no public dataset targets joint tracking and RPM estimation of propeller-like objects. We therefore introduce the Timestamped Quadcopter with Egomotion (TQE) dataset with 13 high-resolution event sequences, containing 52 rotating objects in total, captured at distances of 2 m / 4 m, with increasing egomotion and microsecond RPM ground truth. On TQE, HelixTrack processes full-rate events (approx. 11.8x real time) faster than real time and microsecond latency. It consistently outperforms per-event and aggregation-based baselines adapted for RPM estimation.

==> fig/datasets.tex <==
%\begin{figure}[ht]
\begin{tabular}{|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|@{}c@{}|}
\hline
\includegraphics[width=0.1975\linewidth]{img/dist02_rec1_10160000.png} & \includegraphics[width=0.1975\linewidth]{img/dist02_rec2_26360000.png} & \includegraphics[width=0.1975\linewidth]{img/dist02_rec3_15080000.png} & \includegraphics[width=0.1975\linewidth]{img/dist02_rec4_23320000.png} & \includegraphics[width=0.1975\linewidth]{img/dist02_rec5_15520000.png}  \\
\hline
\includegraphics[width=0.1975\linewidth]{img/dist04_rec1_18480000.png} & \includegraphics[width=0.1975\linewidth]{img/dist04_rec2_15320000.png} & \includegraphics[width=0.1975\linewidth]{img/dist04_rec3_17840000.png} & \includegraphics[width=0.1975\linewidth]{img/dist04_rec4_8480000.png} & \includegraphics[width=0.1975\linewidth]{img/dist04_rec5_13640000.png}  \\
\hline
\end{tabular}
\caption{\tquadcopterego{}}

==> fig/ego_dataset_sampled.tex <==
% \begin{figure}[ht]
\renewcommand{\arraystretch}{0}\centering
\begin{tabular}{*{5}{|@{}c@{}}|}
\hline
\includegraphics[width=0.1975\linewidth]{img/dist2_rec1_11000000.png} & \includegraphics[width=0.1975\linewidth]{img/dist2_rec1_12000000.png} & \includegraphics[width=0.1975\linewidth]{img/dist2_rec1_13000000.png} & \includegraphics[width=0.1975\linewidth]{img/dist2_rec1_14000000.png} & \includegraphics[width=0.1975\linewidth]{img/dist2_rec1_15000000.png}  \\[-1em]
\multicolumn{5}{l}{$M_\text{ego} = 1$} \\
\hline
\includegraphics[width=0.1975\linewidth]{img/dist2_rec7_24000000.png} & \includegraphics[width=0.1975\linewidth]{img/dist2_rec7_25000000.png} & \includegraphics[width=0.1975\linewidth]{img/dist2_rec7_26000000.png} & \includegraphics[width=0.1975\linewidth]{img/dist2_rec7_27000000.png} & \includegraphics[width=0.1975\linewidth]{img/dist2_rec7_28000000.png}  \\[-1em]
\multicolumn{5}{l}{$M_\text{ego} = 7$} \\
\hline
\end{tabular}


==> fig/tracklets.tex <==
\renewcommand{\arraystretch}{0}\centering
\begin{tabular}{*{5}{|@{}c@{}}|}
\hline
\includegraphics[width=0.1975\linewidth]{img/helixtrack_final_states/dist2_rec1.h5.png} & 
\includegraphics[width=0.1975\linewidth]{img/helixtrack_final_states/dist2_rec2.h5.png} & 
%\includegraphics[width=0.1625\linewidth]{img/helixtrack_final_states/dist2_rec3.h5.png} &
\includegraphics[width=0.1975\linewidth]{img/helixtrack_final_states/dist4_rec1.h5.png} & 
\includegraphics[width=0.1975\linewidth]{img/helixtrack_final_states/dist4_rec2.h5.png} & 
\includegraphics[width=0.1975\linewidth]{img/helixtrack_final_states/dist4_rec4.h5.png} \\[-1em]
$d=2\,\mathrm{m},M_\text{ego}=1$ & $d=2\,\mathrm{m},M_\text{ego}=2$ & $d=4\,\mathrm{m},M_\text{ego}=1$ & $d=4\,\mathrm{m},M_\text{ego}=2$ & $d=4\,\mathrm{m},M_\text{ego}=4$ \\
\hline
\end{tabular}

==> tab/benchmark.tex <==
\centering
%\setlength{\tabcolsep}{2pt}
%\fontsize{9.6pt}{11.3pt}\selectfont
\begin{tabular}{ c c r@{ $\pm$ }l r@{ $\pm$ }l r@{ $\pm$ }l r@{ $\pm$ }l c c r}
\toprule
& & \multicolumn{4}{c}{\centering \helixtrack{}} & \multicolumn{4}{c}{AEB-Tracker~\cite{wang_asynchronous_2024}} & \multicolumn{2}{c}{DeepEv~\cite{messikommer_data-driven_2025}} & \\
\cmidrule(r){3-6}\cmidrule(r){7-10}\cmidrule{11-12}
$d$ & $M_{\text{ego}}$  & $\mu_\text{rel}$ & $\sigma_\text{rel}$ & $\mu_\text{RPM}$ & $\sigma_\text{RPM}$ & $\mu_\text{rel}$ & $\sigma_\text{rel}$  & $\mu_\text{RPM}$ & $\sigma_\text{RPM}$ & \hspace{0.3em}$\mu_\text{rel}\pm\sigma_\text{rel}$\hspace{0.3em} & $\mu_\text{RPM}\pm\sigma_\text{RPM}$ & $l$ (s) \\
\midrule
$2$ m  & 1 &  1.3 & 0.1 & 92.8 & 18.4 &  40.8 & 14.9 & 3547.9 & 2801.3 & $F$ & $F$ & 28.7 \\
$2$ m  & 2 &  1.3 & 0.1 & 90.1 & 16.9 &  34.4 & 11.7 & 2465.5 & 1898.2 & $F$ & $F$ & 27.7 \\
$2$ m  & 3 &  10.5 & 7.1 & 680.2 & 974.8 &  \multicolumn{2}{c}{$F$} &  \multicolumn{2}{c}{$F$} & $F$ & $F$ & 27.7 \\
$2$ m  & 4 &  77.0 & 1.8 & 7212.5 & 332.2 &  \multicolumn{2}{c}{$F$} &  \multicolumn{2}{c}{$F$} & $F$ & $F$ & 28.9 \\
$2$ m  & 5 &  81.4 & 10.3 & 7488.4 & 2162.5 &  \multicolumn{2}{c}{$F$} &  \multicolumn{2}{c}{$F$}  & $F$ & $F$ & 28.8 \\
$2$ m  & 6 &  84.4 & 9.2 & 7981.4 & 1705.1 &  \multicolumn{2}{c}{$F$} &  \multicolumn{2}{c}{$F$}  & $F$ & $F$ & 28.1 \\
$2$ m  & 7 &  84.8 & 11.5 & 6497.4 & 1534.1 &  \multicolumn{2}{c}{$F$} &  \multicolumn{2}{c}{$F$}  & $F$ & $F$ & 28.6 \\
$4$ m  & 1 &  19.3 & 18.0 & 1721.3 & 3263.3 &  \multicolumn{2}{c}{$F$} &  \multicolumn{2}{c}{$F$}  & $F$ & $F$ & 28.7 \\
$4$ m  & 2 &  23.8 & 22.4 & 2210.2 & 4233.9 &  57.5 & 10.1 & 4564.7 & 1361.7 &  $F$ & $F$ & 28.2 \\
$4$ m  & 3 &  38.3 & 21.5 & 3449.3 & 3961.3 &  112.1 & 63.8 & 8826.3 & 8395.5 & $F$ & $F$ & 27.9 \\
$4$ m  & 4 &  21.8 & 20.6 & 2152.1 & 4126.9 &  \multicolumn{2}{c}{$F$} &  \multicolumn{2}{c}{$F$}  & $F$ & $F$ & 28.7 \\
$4$ m  & 5 &  69.8 & 22.8 & 6969.1 & 4582.9 &  \multicolumn{2}{c}{$F$} &  \multicolumn{2}{c}{$F$}  & $F$ & $F$ & 27.2 \\
$4$ m  & 6 &  62.9 & 3.0 & 6132.7 & 842.3 &  \multicolumn{2}{c}{$F$} &  \multicolumn{2}{c}{$F$}  & $F$ & $F$ & 28.8 \\
%\midrule
 %\multicolumn{2}{l}{\raisebox{0.15em}{\scalebox{0.8}{$\downarrow$}} \textbf{AVG}} &  \bfseries 44.3 & \bfseries 11.2 & \bfseries 4052.1 & \bfseries 2135.0 & \multicolumn{2}{c}{$F$} & \multicolumn{2}{c}{$F$} & $F$ & $F$ \\
\bottomrule
\end{tabular}

==> tab/benchmark_shortened.tex <==
\centering
% \setlength{\tabcolsep}{2pt}
\newcommand{\grayc}{\color{lightgray}}
\fontsize{9.0pt}{10.0pt}\selectfont
\begin{tabular}{ c @{ } c c r@{ }l r r @{\hspace{1em}} r r @{\hspace{1em}} r @{\hspace{1em}} r r @{\hspace{1em}} r r}
\toprule
& & & & & \multicolumn{3}{c}{\helixtrack{}} & \multicolumn{3}{c}{AEB-Tracker~\cite{wang_asynchronous_2024}} & \multicolumn{3}{c}{DeepEv~\cite{messikommer_data-driven_2025}} \\
\cmidrule(l){6-8}\cmidrule(l){9-11}\cmidrule(l){12-14}
 & &  & & & MArE & MAE & RMSE & MArE & MAE & RMSE & MArE & MAE & RMSE  \\
$d$ & $M_{\text{ego}}$ & $l$ (s) & \multicolumn{2}{c}{propeller} & ($\%$) $\downarrow$ & (RPM) & (RPM) & ($\%$) $\downarrow$ & (RPM) & (RPM) & ($\%$) $\downarrow$ & (RPM) & (RPM)  \\
\midrule
\multirow{12}*{$2$ m\hspace{0.3em}} & \multirow{4}*{1} & \multirow{4}*{28.7} & rear & right & \bfseries 1.3 & \grayc{} 93.7 & \grayc{} 215.9 & 61.4 & \grayc{} 5980.8 & \grayc{} 7186.8 & 8564.8 & \grayc{} 652423.7 & \grayc{} 785896.2 \\
 & & & rear & left & 1.3 & \grayc{} 81.4 & \grayc{} 241.4 & \bfseries 0.9 & \grayc{} 73.0 & \grayc{} 241.2 & 402.4 & \grayc{} 32090.3 & \grayc{} 46466.0 \\
 & & & front & left & \bfseries 1.5 & \grayc{} 118.4 & \grayc{} 194.1 & 35.3 & \grayc{} 2487.0 & \grayc{} 3302.9 & 4132.0 & \grayc{} 303141.3 & \grayc{} 359054.3 \\
 & & & front & right & \bfseries 1.2 & \grayc{} 77.8 & \grayc{} 186.3 & 65.5 & \grayc{} 5650.8 & \grayc{} 7673.3 & 94.6 & \grayc{} 8759.2 & \grayc{} 9700.4 \\
\cmidrule{2-14} 
 & \multirow{4}*{3} & \multirow{4}*{27.7} & rear & right & \bfseries 1.2 & \grayc{} 85.1 & \grayc{} 223.2 & 1198.7 & \grayc{} 102482.5 & \grayc{} 192935.8 & 5013.6 & \grayc{} 386360.6 & \grayc{} 437954.9 \\
 & & & rear & left & 31.7 & \grayc{} 2137.8 & \grayc{} 4518.8 & \bfseries 15.0 & \grayc{} 1696.4 & \grayc{} 3482.9 & 2059.8 & \grayc{} 151319.8 & \grayc{} 184206.2 \\
 & & & front & left & \bfseries 4.2 & \grayc{} 230.2 & \grayc{} 763.8 &  467.5 & \grayc{} 37691.4 & \grayc{} 81016.3 & 5236.2 & \grayc{} 376231.1 & \grayc{} 448776.7 \\
 & & & front & right & \bfseries 4.8 & \grayc{} 267.9 & \grayc{} 1031.9 &  1347.9 & \grayc{} 110056.2 & \grayc{} 202948.8 & 195.7 & \grayc{} 14595.8 & \grayc{} 18910.5 \\
\cmidrule{2-14}
 & \multirow{4}*{5}& \multirow{4}*{28.8} & rear & right & \bfseries 62.3 & \grayc{} 6347.2 & \grayc{} 7842.7 & 531.3 & \grayc{} 41415.3 & \grayc{} 79321.0 & 106.7 & \grayc{} 9244.0 & \grayc{} 10241.1 \\
 & & & rear & left & \bfseries 100.9 & \grayc{} 9689.7 & \grayc{} 10899.5 &  480.0 & \grayc{} 30491.9 & \grayc{} 67097.7 & 117.9 & \grayc{} 10624.2 & \grayc{} 12239.0 \\
 & & & front & left & \bfseries 65.0 & \grayc{} 5045.3 & \grayc{} 6266.7 &  389.8 & \grayc{} 33458.3 & \grayc{} 69659.2 & 99.3 & \grayc{} 8963.0 & \grayc{} 9836.3 \\
 & & & front & right & \bfseries 97.7 & \grayc{} 8871.4 & \grayc{} 9710.6 & 1122.0 & \grayc{} 77151.0 & \grayc{} 111267.4 & 398.5 & \grayc{} 32523.2 & \grayc{} 56823.0 \\
\midrule
\multirow{12}*{$4$ m\hspace{0.3em}} & \multirow{4}*{1} & \multirow{4}*{28.7} & rear & right & \bfseries 73.1 & \grayc{} 6616.3 & \grayc{} 8517.8 & 285.5 & \grayc{} 21029.7 & \grayc{} 46759.1 & 834.5 & \grayc{} 57801.3 & \grayc{} 73901.3 \\
 & & & rear & left & \bfseries 1.2 & \grayc{} 76.4 & \grayc{} 158.4 & 57.2 & \grayc{} 6038.7 & \grayc{} 20115.0 & 89.6 & \grayc{} 8341.9 & \grayc{} 9422.8 \\
 & & & front & left & \bfseries 1.4 & \grayc{} 104.8 & \grayc{} 255.3 & 48.9 & \grayc{} 4676.4 & \grayc{} 16769.4 & 88.7 & \grayc{} 7853.7 & \grayc{} 8925.9 \\
 & & & front & right & \bfseries 1.3 & \grayc{} 87.8 & \grayc{} 319.4 & 165.4 & \grayc{} 13041.8 & \grayc{} 36853.1 & 835.4 & \grayc{} 58054.3 & \grayc{} 74833.5 \\
\cmidrule{2-14}
 & \multirow{4}*{3} & \multirow{4}*{28.9} & rear & right & 70.9 & \grayc{} 5770.0 & \grayc{} 7008.1 & \bfseries 58.8 & \grayc{} 5904.9 & \grayc{} 11479.0 & 95.8 & \grayc{} 9773.3 & \grayc{} 10725.7 \\
 & & & rear & left & \bfseries 1.3 & \grayc{} 85.0 & \grayc{} 211.7 & 46.8 & \grayc{} 3960.0 & \grayc{} 4845.4 & 1801.4 & \grayc{} 140787.4 & \grayc{} 181653.8 \\
 & & & front & left & \bfseries 1.3 & \grayc{} 109.4 & \grayc{} 210.8 & 303.1 & \grayc{} 21349.0 & \grayc{} 51357.9 & 1937.2 & \grayc{} 146814.9 & \grayc{} 174482.0 \\
 & & & front & right & 79.8 & \grayc{} 7832.8 & \grayc{} 9394.6 \grayc{} & \bfseries 39.7 & \grayc{} 4091.3 & \grayc{} 5306.3 & 97.4 & \grayc{} 9594.5 & \grayc{} 10465.4 \\
\cmidrule{2-14}
 & \multirow{4}*{5} & \multirow{4}*{27.2} & rear & right & \bfseries 95.3 & \grayc{} 9688.6 & \grayc{} 10614.2 & 994.6 & \grayc{} 83816.5 & \grayc{} 127547.1 & 97.8 & \grayc{} 9942.3 & \grayc{} 10817.5 \\
 & & & rear & left & \bfseries 93.9 & \grayc{} 9316.3 & \grayc{} 10400.6 & 1043.3 & \grayc{} 76882.9 & \grayc{} 133235.2 & 94.8 & \grayc{} 9332.0 & \grayc{} 10351.1 \\
 & & & front & left & \bfseries 1.7 & \grayc{} 119.1 & \grayc{} 241.1 & 1092.8 & \grayc{} 81598.8 & \grayc{} 126119.1 & 3339.1 & \grayc{} 260136.5 & \grayc{} 310936.4 \\
 & & & front & right & \bfseries 88.3 & \grayc{} 8752.7 & \grayc{} 9711.9 & 1126.9 & \grayc{} 93336.6 & \grayc{} 134050.9 & 95.6 & \grayc{} 9351.7 & \grayc{} 10281.2 \\
\bottomrule
\end{tabular}

==> tab/dataset_statistics.tex <==

\begin{table}[h!]
\centering
\begin{subtable}[t]{1\columnwidth}
\centering
\begin{tabular}{l r r r r r}
\toprule
DS & $|\text{DS}|$ & min & max & avg & med \\
\midrule
%\multicolumn{8}{c}{\tpropeller{}}\\
%\midrule
  %TP & 5 & 63.2 & 64.5 & 63.8 & 63.8  \\
 %\midrule
 %\multicolumn{8}{c}{\tquadcopter{}}\\
 %\midrule
 %TQ & 37 & 12.7 & 75.5 & 20.1 & 18.0 \\
%\midrule
%\multicolumn{8}{c}{\tquadcopterego{}}\\
%\midrule
  TQE & 13 & 33.3 & 35.0 & 34.3 & 34.5  \\
\bottomrule
\end{tabular}
\caption{Duration of recordings (s)}
\label{tab:dataset_statistics_durations}
\end{subtable}

\begin{subtable}[t]{1\columnwidth}
\centering
\begin{tabular}{l r r r r}
\toprule
DS &  min & max & avg & med \\
\midrule
%\multicolumn{8}{c}{\tpropeller{}}\\
%\midrule
  %TP  & 9773 & 9804 & 9782.4 & 9778 \\
 %\midrule
 %\multicolumn{8}{c}{\tquadcopter{}}\\
 %\midrule
 %TQ & 381 & 10413 & 2266.7 & 2165 \\
%\midrule
%\multicolumn{8}{c}{\tquadcopterego{}}\\
%\midrule
  TQE & 4770 & 5116 & 4906.5 & 4876 \\
\bottomrule
\end{tabular}
\caption{Number of ground-truth timestamps}
\label{tab:dataset_statistics_timestamps}
\end{subtable}
\caption{Overview of dataset statistics for the evaluation \tquadcopterego{} dataset (\tquadcopteregoshort{}). Table (a) presents the duration of recordings (in seconds), detailing the number of recordings ($|\text{DS}|$) along with minimum, maximum, average, and median values. Table (b) reports the number of timestamps in the ground-truth per recording, including minimum, maximum, average, and median counts.}\label{tab:dataset_statistics}
\end{table}
